Universal Barrier Functions for Safety and Stability of Constrained Nonlinear Systems

In this paper, we address the problem of synthesizing safe and stabilizing controllers for nonlinear systems subject to complex safety specifications and input constraints. We introduce the Universal Barrier Function (UBF), a single continuously differentiable scalar-valued function that encodes both stability and safety criteria while accounting for input constraints. Using the UBF, we formulate a Quadratic Program (UBF-QP) to generate control inputs that are both safe and stabilizing under input constraints. We demonstrate that the UBF-QP is feasible if a UBF exists. Furthermore, under mild conditions, we prove that a UBF always exists. The proposed framework is then extended to systems with higher relative degrees. Finally, numerical simulations illustrate the effectiveness of our proposed approach.

==> packages.tex <==
\usepackage{times}
\usepackage{float}
\usepackage{hyperref}
\usepackage{algorithmic}
\usepackage{subcaption}
\usepackage{xcolor}
\usepackage{graphicx}
\usepackage{adjustbox}
\usepackage{multirow}
\usepackage{pbox}
\usepackage{algorithm}
\usepackage{amsmath} 
% \usepackage{amsthm}
\usepackage{natbib}
\usepackage{pgfplotstable} % Ensure this package is included

% \usepackage{aliases}
% \defbibalias{marley2024hybrid_systems_1_alias}{marley2024hybrid_systems_1}

\usepackage{csvsimple}
% \usepackage{tikz}
 % \usepackage{algpseudocode}
\usepackage{pgfplots}
\usepgfplotslibrary{external}
\tikzexternalize[prefix=figures/]
\usepgfplotslibrary{contour}
\newcommand{\ed}{{\boldsymbol{e}_d}}
% \usepgfplotslibrary{groupplots,dateplot}
% \usetikzlibrary{patterns,shapes.arrows}
% \pgfplotsset{compat=newest}
\usepackage{hyperref}

\usepackage{adjustbox}
 \usepackage{multirow}
% \usepackage{multicol}
\usepackage{pbox}
% \usepackage{minipage}
% \usepackage{tikz}
% \usetikzlibrary{shapes, arrows.meta, positioning}

% \usepgfplotslibrary{groupplots}
% \usepgfplotslibrary{fillbetween}
% \usetikzlibrary{arrows,decorations.pathmorphing,positioning,fit,trees,shapes,shadows,automata,calc} 
% \usetikzlibrary{patterns,arrows,arrows.meta,calc,shapes,shadows,decorations.pathmorphing,decorations.pathreplacing,automata,shapes.multipart,positioning,shapes.geometric,fit,circuits,trees,shapes.gates.logic.US,fit, matrix,arrows.meta, quotes}
% \usetikzlibrary{backgrounds,scopes}
% \usepackage{ulem}
% \usepackage{amsfonts}
% \usepackage{tabu}

\newtheorem{problem}{Problem}
% \newtheorem{prop}{Proposition}
% \newtheorem{step}{Step}
\newtheorem{remark}{Remark}
\newtheorem{lemma}{Lemma}
\newtheorem{corollary}{Corollary}
\newtheorem{definition}{Definition}
\newtheorem{assumption}{Assumption}
\newtheorem{theorem}{Theorem}
\newtheorem{example}{Example}
% \newtheorem{proof}{Proof}
% Define an unnumbered proof environment
% \newenvironment{proof}%
%     {\par\noindent{\bf Proof}\hspace{1em}} % This line sets up the environment
%     {\hfill$\square$} % This line ends the environment


% % Theorem environments
% \theoremstyle{plain}
% \newtheorem{theorem}{Theorem}[section]
% \theoremstyle{definition}
% \newtheorem{definition}{Definition}
% \theoremstyle{remark}
% \newtheorem{remark}{Remark}

==> tikz/sets.tex <==
% Draw a smooth closed curve
  \begin{scope}[shift={(-3,5.5)}, scale=1.6, ]
    \draw[thick, black, fill=green!30, fill opacity=0.5] 
      plot[smooth cycle, tension=.7] coordinates{(1,-1) (3,0) (4,-2) (2.5,-3) (-0.5,-2)};
  \end{scope}
% \draw[thick, black, fill=green, fill opacity=0.5] 
  % plot[smooth cycle, tension=.7] coordinates{(1,-1) (3,0) (4,-2) (2.5,-3) (-0.5,-2)};
  \begin{scope}[shift={(0.5,0)}, scale=1.2]
  \draw[thick, black, fill=blue!30, fill opacity=0.5] 
  plot[smooth cycle, tension=.7] coordinates{(-1,3) (1,3) (2,3) (0.5,1) (-2.5,2)};
  \end{scope}

    \begin{scope}[shift={(0.2,0.85)}, scale=0.6, rotate=135]
    \draw[thick, black, fill=red!30, fill opacity=0.5] 
      plot[smooth cycle, tension=.7] coordinates{(1,-1) (3,0) (4,-2) (2.5,-3) (-0.5,-2)};
  \end{scope}

% % Add text inside the curve
 \node at (1, 4.5) {$\mathcal{S}_V$};
\node at (1.5, 3) {$\mathcal{A}_s$};

% Draw an arrow from inside to outside
% \draw[thick,->] (1.5, -1.0) -- (0, -0.5);

% Add text outside the curve
% \node at (-0.5, 0.3) {$\mathcal{K}_{\text{CBF}}=\{\bu\in\mathbb{R}^m\;|\;\dot{h}(\bx)\geq -\alpha(h(\bx))\}$};
